Distributing Content Simplifies ISP Traffic Engineering

Several major Internet service providers (e.g., Level-3, AT&T, Verizon) today also offer content distribution services. The emergence of such "Network-CDNs" (NCDNs) are driven by market forces that place more value on content services than just carrying the bits. NCDNs are also necessitated by the need to reduce the cost of carrying ever-increasing volumes of traffic across their backbones. An NCDN has the flexibility to determine both where content is placed and how traffic is routed within the network. However NCDNs today continue to treat traffic engineering independently from content placement and request redirection decisions. In this paper, we investigate the interplay between content distribution strategies and traffic engineering and ask how an NCDN should engineer traffic in a content-aware manner. Our experimental analysis, based on traces from a large content distribution network and real ISP topologies, shows that effective content placement can significantly simplify traffic engineering and in most cases obviate the need to engineer NCDN traffic all together! Further, we show that simple demand-oblivious schemes for routing and placement such as InverseCap and LRU suffice as they achieve network costs that are close to the best possible.

==> Conclusions.tex <==
\section{Conclusions}
\label{sec:concl}


We posed and studied the content-aware traffic engineering problem where content distribution and traffic engineering decisions are optimized jointly as opposed to being optimized separately as is done today. This paradigm is of key importance to \ncp s who own and manage the infrastructure for content distribution as well as the underlying network. Our trace-driven experiments using extensive access logs from the world's largest CDN and real ISP topologies resulted in the following key conclusions. First, simple demand-oblivious schemes for routing and placement, such as InverseCap and LRU, outperformed sophisticated placement and routing schemes computed once-a-day based on the prior day's demand. Second,  traffic demand can be ``shaped'' by effective content placement to the extent that the effectiveness of traditional traffic engineering is marginalized.  Finally, we studied the value of the future knowledge of demand for placement and routing decisions. While future knowledge helps, what is perhaps surprising is that a small amount of additional storage and simple optimizations such as content chunking and link-utilization-aware redirection allows simple, demand-oblivious schemes to perform as well as demand-aware ones with future knowledge.


==> RelatedWork-alt.tex <==
%\section{Discussion}
%\label{sec:limitations}

\textbf{A note on the need for traffic engineering:} Overall, our results suggest that optimizing routing yields little improvement to network cost for the NCDN portion of the traffic, but this finding does not imply that traffic engineering by ISPs is unnecessary. ISPs route transit traffic in addition to NCDN traffic, and they do not control either content placement or request redirection for transit traffic, therefore, traditional traffic engineering methods, e.g., OSPF traffic engineering, can reduce the network cost due to transit traffic. The benefit of traffic engineering, or lack thereof, depends on the fraction of transit traffic vs. NCDN traffic in an ISP.

%Our results suggest that optimizing routing yields little improvement to network cost for the NCDN portion of the traffic, but this finding does not imply that traffic engineering by ISPs is unnecessary. An important reason for ISPs to engineer traffic is that they route transit traffic in addition to NCDN traffic. Since an ISP does not control either content placement or request redirection for transit traffic, traditional traffic engineering methods, e.g., OSPF traffic engineering, can reduce the network cost due to transit traffic. The benefit of traffic engineering, or lack thereof, depends on the fraction of transit traffic vs. NCDN traffic in an ISP. 


%\textbf{How does dynamic content impact this analysis?} Dynamic content is outside the scope of this work. That said, it contributes to a much smaller volume of traffic compared to static content such as on-demand video and downloads, so an NCDN is likely to achieve the most significant reduction in network cost by focusing just on static content.

%\textbf{Does end-user performance not affect 
%How does dynamic content impact your analysis?} An NCDN may additionally consider end-user performance, not just the network cost, while deciding placement and routing. We plan to consider the effectiveness 

\eat{
(1) Our \ncp\ model models only the CDN traffic and not the transit traffic which present in an ISP network. Since, an ISP cannot control content placement for transit traffic, traffic engineering will help reduce network cost for transit traffic.

(2) Minimizing network cost in face of link failures, either planned or accidental, is one of the goals of traffic engineering. \Ancp\ could suffer from link failures as well as server failures at the PoPs. We intend to study the effect of link failures as well as server failures for \ancp\ in our future work.
}


\section{Related Work}
\label{sec:related}

Traffic engineering and content distribution have both seen an enormous body of work over more than a decade. To our knowledge, our work is the first to pose the \ncp\ problem, wherein a single entity seeks to address both concerns, and empirically evaluate different content-aware traffic engineering strategies. 
%\noindent\textbf{Interaction of location diversity and TE:}



\textbf{Joint optimization:} Recent work has explored the joint optimization of traffic engineering and ``content distribution'', where the latter term refers to the {\em server selection} problem. P4P (Xie et al.  \cite{P4P}) shows that P2P applications can improve their performance and ISPs can reduce the MLU and interdomain costs, if P2P applications adapt their behavior based on hints supplied by ISPs. Jiang et al.  \cite{Jiang2009} and  DiPalantino et al. \cite{JohariGameTheory} both study the value of joint optimization of traffic engineering and content distribution versus   independent optimization of each. CaTE (Frank at al. \cite{cate}),  like P4P, shows that a joint optimization can help both ISPs and content providers improve their performance. These works equate content distribution to server selection (or request redirection in our parlance), while the NCDN problem additionally considers content placement itself as a degree of freedom. As our results show, optimizing placement is powerful and can single-handedly reduce the MLU significantly even in conjunction with simple request redirection and routing strategies.

%CaTE \cite{cate},  like P4P,  shows that both ISPs and content providers can benefit if content providers perform request redirection based on network information provided by ISPs. 

% supply hints  to P2P (called as \emph{p-distances}) applications, and the 

%that ISP should supply hints  to P2P applications that when used by them improves their performance and also reduces interdomain transit costs and the MLU for the ISP.  




%interaction between traffic engineering and content distribution using a game-theoretic model and show that, without a joint optimization, the equilibrium of this interaction may not result in a socially optimal solution.  

%Jiang et al.  \cite{Jiang2009} and  DiPalantino et al. \cite{JohariGameTheory} both study the interaction between traffic engineering and content distribution using a game-theoretic model and show that, without a joint optimization, the equilibrium of this interaction may not result in a socially optimal solution.  


%\noindent\textbf{Content Placement in ISP networks:}
% content pl
%\noindent\textbf{Network CDNs:}
%Major ISP/Telco organizations such as AT \& T \cite{att-cdn}, Level-3 \cite{level3-cdn}and Verizon \cite{verizon-cdn} are building hosting and content delivery infrastructure into their networks.  ISPs enjoy a natural advantage for a CDN since they can place content within their networks at close proximity to their own customers. ISPs can integrate CDN infrastructure such as storage and server clusters at their PoP locations. The falling prices of bandwidth are providing the push to these companies to enter CDN market. 

\textbf{Placement optimization:}
Applegate et al. \cite{Applegate2010} study the content placement problem for a VoD system that seeks to minimize the aggregate network bandwidth consumed. However, they assume a {\em fixed routing} in the network, while one of our contributions is to assess the relative importance of optimizing routing and optimizing  placement in an NCDN.

%  There are two key differences between their work and ours. First, they assume a {\em fixed routing} in the network, while one of our contributions is to assess the relative importance of optimizing routing and optimizing  placement in an NCDN. Second, 


Furthermore, they find that an optimized, demand-aware placement with a small local cache (similar to our ``hybrid'' strategy in $\S$\ref{sec:hybrid}) outperforms LRU. In contrast, our experiments suggest otherwise. There are three explanations for this disparity. First,  their workload seems to be predictable even at weekly time scales, whereas the Akamai CDN traces that we use show significant daily churn.  Second, their scheme has some benefit  of future knowledge and is hence somewhat comparable to our \optrpfuture. For a large \ncp, obtaining knowledge about future demand may not be practical for all types of content, e.g., breakout news videos. Finally,  our analysis suggests that LRU performs sub-optimally only at small storage ratios,  and the difference between  LRU and \optrpfuture\ reduces considerably at higher storage ratios (not considered in \cite{Applegate2010}).


\eat{
The disparity in the performance of demand-aware schemes  observed in \cite{Applegate2010} and in our experiments can be explained as follows: (1) Their workload seems to predictable even at weekly time scales, while our CDN traces consisting of a variety of on-demand video and downloads traffic exhibit significant daily churn. (2) Their scheme has some benefit  of future knowledge and is hence somewhat comparable to the \optrpfuture\ scheme. For a large \ncp, obtaining knowledge about future demand may not be practical for all types of content, e.g., news videos. (3) Our analysis suggests that LRU performs worse only at small storage ratios,  and the difference between  LRU and optimized placement  reduces considerably on increasing the storage ratio.
}

% They  compare different video placement algorithms and find that an optimized, demand-aware placement strategy with a small local cache (similar to our ``hybrid'' strategy in $\S$\ref{sec:hybrid}) outperforms purely demand-oblivious LRU-like strategies. Our work differs from theirs with respect to both the problem addressed and the qualitative findings as follows. We model an \ncp\ that in addition to placement also controls routing, and assessing the relative importance of routing and placement strategies is one of our contributions. 




%Furthermore, unlike \cite{Applegate2010}, we find that a simple, demand-oblivious, LRU strategy significantly outperforms an optimized, demand-aware (static or hybrid) placement strategy. There are a explanations for this seeming disparity. First, we consider a comprehensive trace of CDN requests with a variety of on-demand video as well as download traffic that exhibits significant daily churn; in comparison, their workload appears to be reasonably predictable even over weekly timescales. Second, the optimized, demand-aware placement strategy they consider also has some benefit of future knowledge and is therefore somewhat comparable to a demand-aware scheme with future knowledge (\optrpfuture\ in $\S$\ref{sec:eval}). In general, obtaining knowledge about future demand may not be practical for all types of content, e.g., news videos, for a large \ncp.  Furthermore, our analysis of different storage ratios suggests that LRU performs worse only at small storage ratios,  and the difference between  LRU and optimized content placement reduces significantly on increasing the storage ratio.


\textbf{Traffic engineering:} Several classes of traffic engineering schemes such as OSPF link-weight optimization \cite{fortz2000internet}, MPLS flow splitting \cite{MPLS2},  optimizing routing for multiple traffic matrices \cite{COPE, multiTM}, online engineering \cite{TEXCP,MPLS2}, and oblivious routing \cite{Cohen,Racke}, have been studied. All of these schemes assume that the demand traffic is a given to which routing must adapt. However, we find that \ancp\ is in a powerful position to change the demand traffic matrix, so much so that even a naive scheme like InverseCap, i.e., no engineering at all, suffices in conjunction with a judicious placement strategy and optimizing routing further adds little value. In this respect, our findings are comparable in spirit to Sharma et al. \cite{Abhigyan}. However, they focus on the impact of location diversity, and show that even a small, fixed number of randomly placed replicas of each content suffice to  blur differences between different engineering schemes with respect to a capacity metric (incomparable to MLU), but find that engineering schemes still outperform InverseCap routing.

%OSPF, MPLS based schemes, online schemes. these schemes are based on a notion of traffic matrix which is known apriori. in our model traffic matrix is not fixed but it depends on the content placement and flow split in the network. Our work compares the performance of naive traffic engineering InvCap and Optimal traffic engineering in a network for a variety of content placement and flow split strategies. we arrive at the conclusion that traditonal traffic engineering makes little different when content placement and flow split is optimized in the network.

%\noindent\textbf{Facility Location:} \tbd{Ramesh: do you want to write something here?}



